(Chat)GPT v BERT: Dawn of Justice for Semantic Change Detection

In the universe of Natural Language Processing, Transformer-based language models like BERT and (Chat)GPT have emerged as lexical superheroes with great power to solve open research problems. In this paper, we specifically focus on the temporal problem of semantic change, and evaluate their ability to solve two diachronic extensions of the Word-in-Context (WiC) task: TempoWiC and HistoWiC. In particular, we investigate the potential of a novel, off-the-shelf technology like ChatGPT (and GPT) 3.5 compared to BERT, which represents a family of models that currently stand as the state-of-the-art for modeling semantic change. Our experiments represent the first attempt to assess the use of (Chat)GPT for studying semantic change. Our results indicate that ChatGPT performs significantly worse than the foundational GPT version. Furthermore, our results demonstrate that (Chat)GPT achieves slightly lower performance than BERT in detecting long-term changes but performs significantly worse in detecting short-term changes.

==> main_backup.tex <==
\section{Introduction}
Lexical semantic change is the computational study of how words change their meanings over time~\cite{montanelli2023survey,nina2021survey,kutuzov2018diachronic}. These changes are crucial to our understanding of historical and general out-of-domain texts. Indeed, a nuanced grasp of semantic \textit{variation} between groups, or semantic \textit{change} across time, allows us to study languages, cultures and societies through digitized text and open up a range of research applications. As such, computational approaches to semantic change are necessary tools for a range of other research fields with immense potential: from broadening historical linguistics and simplifying lexicography, to studies in sociology, history, medicine, and other text-based sciences. These approaches include both the computational representation of word meaning as well as the detection of change. Critically, the study of semantic change can also serve as an important method to evaluate the true capacity for generalization of large language models, as it serves as a litmus test of their ability to handle text under unique out-of-distribution (OOD) conditions.

The recent introduction of Transformers-based language models has led to significant advancements in Natural Language Processing (NLP)~\cite{Vaswani2017attention}. These advancements are exemplified in Pretrained Foundation Models (PFMs) like BERT~\cite{devlin2019bert} and ChatGPT~\footnote{\url{chat.openai.com}}, which ``\textit{are regarded as the foundation for various downstream tasks}''~\cite{zhou2023comprehensive}.  BERT has experienced a surge in popularity over the last years and BERT-based methods have repeatedly provided state-of-the-art (SOTA) results for computational modeling of semantic change~\cite{montanelli2023survey,cassotti2023xl}. However, research focus is now shifting towards ChatGPT due to its impressive ability to generate fluent and high-quality responses to human queries, 
% CAMERA READY: mention GPT paper at LChange
making it the fastest-growing AI tool to amass 100 million users. Recently, several research works have assessed the language capabilities of ChatGPT by using a wide range of prompts to solve popular NLP tasks~\cite{laskar2023systematic,KOCON2023ChatGPT}. However, current evaluations generally (a) overlook that the output of ChatGPT is non-deterministic\footnote{\url{platform.openai.com/docs/guides/gpt/faq}}, and (b) only rely on contemporary and synchronic text. As a result, these evaluations provide valuable insights into the generative, pragmatic and semantic capabilities of ChatGPT~\cite{KOCON2023ChatGPT}, but fall short in assessing its potential for solving OOD tasks, and specifically handling historical and diachronic text, which constitute a unique scenario for testing models' generalization.

In this paper, we propose to evaluate the capability of ChatGPT in recognizing (lexical) \textit{semantic change}, often also referred to as \textit{semantic shift}. Although the Lexical Semantic Change (LSC) evaluation task has recently been proposed in NLP~\cite{schlechtweg2020semeval}, its setup is not suitable for evaluating a model like ChatGPT due to the limited size of ChatGPT's prompts and answers, as well as accessibility limitations such as hourly character limit and economic constraints\footnote{LSC involves identifying words that change meanings over time in a diachronic corpus. Typically, this task is approached by considering all usages of a word across two or more time periods, which can consist of several thousand sentences. These quantities are too large to fit into a ChatGPT prompt.}. In light of these considerations, we therefore evaluate the potential of ChatGPT through the Word-in-Context (WiC) task, which has recently demonstrated a robust connection with LSC~\cite{cassotti2023xl}. In particular, we consider two diachronic extensions of the original WiC setting, namely \textit{temporal} WiC (TempoWiC) and \textit{historical} WiC (HistoWiC). Our goal is to determine if a word carries the same meaning in two different contexts of different time periods, or conversely, those contexts exemplify a semantic change. While TempoWiC has been designed for evaluating PFMs in detecting ``short-term changes'' in social media~\cite{loureiro2022tempowic}, HistoWiC is our adaptation of the %large annotations underlying the 
SemEval-2020 LSC benchmark on historical text to the WiC task for evaluating PFMs in detecting ``long-term changes'' in historical corpora~\cite{schlechtweg2020semeval}.

%CAMERA READY
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.6\columnwidth]{imgs/meme.png}
%\caption{The title of this paper draws inspiration by the movie \textit{Batman v Superman: Dawn of Justice}. In this paper, we leverage the analogy of ChatGPT and BERT, powerful and popular PFMs, as two lexical superheroes often erroneously associated for solving similar problems. Our aim is to shed lights on the potential of ChatGPT and dispel the expanding belief that ChatGPT renders BERT an outdated technology}
%\label{fig:meme}
%\end{figure}

Considering the remarkable performance of contextualized BERT models in addressing WiC and LSC tasks~\cite{montanelli2023survey}
%CAMERA READY: periti2023contextualized,periti2023time
, we compare the performance of ChatGPT in TempoWiC and HistoWiC to those obtained by using BERT. While BERT is specifically designed to understand the meaning of words in contexts, ChatGPT is designed to generate fluent and coherent text. Through these two \textit{lexical superheros}\footnote{The paper is inspired by the movie \textit{Batman v Superman: Dawn of Justice}. We leverage the analogy of ChatGPT and BERT, as two lexical superheroes often erroneously associated}, %CAMERA READY (see Fig~\ref{fig:meme}), 
our intention in this paper is to illuminate the potential of ChatGPT and mark the dawn of a new era by empirically assessing if ChatGPT makes outdated the common approaches to WiC and LSC that rely on similarities among BERT embeddings.

\section{Related work}
The significant attention garnered by ChatGPT has led to a large number of studies being published immediately after its release. Early studies primarily focused on exploring benefits and risks associated with using ChatGPT in expert fields such as education~\cite{lund2023chatting}, medicine~\cite{ANTAKI2023100324}, or business~\cite{Shaji2023Review}. Evaluation studies are currently emerging for assessing the generative and linguistic ChatGPT's capabilities across a wide range of downstream task in both monolingual and multilingual setups~\cite{bang2023multitask,shen2023hugginggpt,lai2023chatgpt}.

Most evaluations involve a limited number of instances for each task considered (e.g. 50,~\citealp{zhong2023chatgpt,alberts2023large,khalil2023chatgpt}). When the official API is used to query ChatGPT, this is due to the hourly token processing limit\footnote{\url{help.openai.com/en/articles/4936856-what-}\\\url{are-tokens-and-how-to-count-them}} and associated costs\footnote{\url{openai.com/pricing}}. When the web interface is used instead of the API, this is due of the time-consuming process of interacting with ChatGPT, which keeps ``humans in the loop''. However, even when systematic and comprehensive evaluations are conducted~\cite{KOCON2023ChatGPT,laskar2023systematic}, they rely on a single experiment for each task. 

While different single experiments provide valuable insights into ChatGPT's capabilities, they fall short in assessing the potential of ChatGPT for solving specific tasks due to its non-deterministic nature.
Therefore, multiple experiments should be conducted to validate its performance on each task, individually. In addition, current  evaluations generally leverage tasks that overlook the temporal dimension of text, leaving a gap in understanding ChatGPT's ability to handle diachronic and historical text.

\paragraph{Our original contribution.}
Our evaluation of ChatGPT focuses on two diachronic extensions of the WiC task, namely TempoWiC and HistoWiC. Our aim is to assess the potential of ChatGPT for \textit{semantic change detection}. To the best of our knowledge, our work is the first to investigate the application of ChatGPT for Historical Linguistics purposes. 

Thus far, the conventional WiC task has been evaluated only by~\citealp{laskar2023systematic,KOCON2023ChatGPT}, who reported low accuracy % of 62.1\% and 64.58\%, 
under a single setup. In this paper, we challenge these performance by considering diachronic text and multiple setup, totaling 47 experiments each for TempoWiC and HistoWiC:
\begin{itemize}
    \item \textbf{ChatGPT prompts}. \ Similar to~\citealp{zhong2023chatgpt}, we evaluate ChatGPT using zero-shot and few-shot prompting strategies, while also exploring many-shot prompting. Our results demonstrate that zero-shot prompting is more effective on HistoWiC, while few-shot prompting is more effective on TempoWiC. 

    \item \textbf{ChatGPT temperature}. \ Similar to~\citealp{peng2023making,liu2023code}, we analyze how ChatGPT's performance varies according to its temperature hyper-parameter, which controls the ``creativity'' or randomness of its answers. Our results indicate that ChatGPT used with low temperature values, i.e., less creativity, is better at handling WiC tasks. 
    
    \item \textbf{ChatGPT API v ChatGPT Web}. \ We empirically assess if ChatGPT produces worse results via the OpenAI API compared to the web interface\footnote{Discussions on this topic are currently very active. E.g.~\url{community.openai.com/t/web-app-vs-api-}\\\url{results-web-app-is-great-api-is-pretty-awful/96238}}. Our results demonstrate that using the official API for addressing WiC tasks is beneficial compared to using ChatGPT through the web interface, as previously done in recent work~\cite{laskar2023systematic,KOCON2023ChatGPT}. Furthermore, our findings suggest that an intermediate temperature is set to prompt ChatGPT through the web interface.

    \item \textbf{ChatGPT v BERT}. \ Finally, similar to~\citealp{zhong2023chatgpt}, we compare the performances of ChatGPT and BERT. By leveraging the TempoWiC task and introducing the novel \textbf{HistoWiC} task, we shed lights on the potential of both models and demonstrate the superiority of BERT in dealing with diachronic text and WiC tasks.
\end{itemize}

\section{Semantic Change Detection}
Our evaluation relies on two diachronic definitions of the conventional Word-in-Context (WiC) task~\cite{pilehvar2019wic}, namely TempoWiC and HistoWiC. WiC is framed as a binary classification problem, where each instance is associated with a target word $w$,  either a verb or a noun, for which two contexts $c_1$ and $c_2$, are provided. The task is to identify whether the occurrences of $w$ in $c_1$ and $c_2$ correspond to the same meaning or not. Similarly, both TempoWiC and HistoWiC rely on the same definition of the task while being specifically designed for semantic change detection in diachronic text.

\subsection{Temporal Word-in-Context}
TempoWiC is designed as an evaluation benchmark for detecting short-term semantic change in social media, where language is extremely dynamic, and NLP models struggle to cope with new content and trends. In particular, TempoWiC uses tweets from different time periods as contexts $c_1$ and $c_2$.

Considering the limits of testing ChatGPT, we follow~\citealp{zhong2023chatgpt,jiao2023chatgpt} and randomly sample a subset of the original TempoWiC datasets. While the original TempoWiC framework provides trial, train, test, and dev sets, here we do not consider the dev set. Table~\ref{tab:datasets} shows the number of positive (i.e., same meaning) and negative (i.e., different meanings due to semantic change) examples we have considered for each set.

\begin{table}[!ht]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{ccccccc}
                                   & \multicolumn{3}{c}{\textbf{TempoWiC}}     & \multicolumn{3}{c}{\textbf{HistoWiC}}     \\ \cline{2-7} 
\multicolumn{1}{c|}{}              & Trial & Train & \multicolumn{1}{c|}{Test} & Trial & Train & \multicolumn{1}{c|}{Test} \\ \cline{2-7} 
\multicolumn{1}{c|}{\textit{True}} & 8     & 86    & \multicolumn{1}{c|}{73}   & 11    & 137   & \multicolumn{1}{c|}{79}   \\
\multicolumn{1}{c|}{\textit{False}} & 12 & 114 & \multicolumn{1}{c|}{127} & \textit{9} & 103 & \multicolumn{1}{c|}{61} \\ \cline{2-7} 
\multicolumn{1}{c|}{\textbf{Tot}}  & 20    & 200   & \multicolumn{1}{c|}{200}  & 20    & 200   & \multicolumn{1}{c|}{140}  \\ \cline{2-7} 
\end{tabular}}
\caption{Datasets used in our evaluation} %CAMERA READY: TempoWiC and HistoWiC datasets used in our evaluation
\label{tab:datasets}
\end{table}

\subsection{Historical Word-in-Context}
We design HistoWiC as a novel evaluation benchmark for detecting long-term semantic change in historical text, where language may vary across different epochs, and NLP models struggle to cope with historical content and trends. HistoWiC sets the two contexts $c_1$ and $c_2$, as sentences collected from the two English corpora of SemEval-2020 LSC detection task ~\cite{schlechtweg2020semeval}. 

Similar to WiC, the annotation process for the LSC benchmark involved usage pair annotations, where a target word is used in two different contexts. Thus, we directly utilize the annotated instances for LSC to develop HistoWiC. Since LSC instances were annotated by using the DURel framework and a semantic relatedness four-point scale~\cite{schlechtweg2020semeval,schlechtweg2018diachronic}, 
%CAMERA READY(see Table~\ref{tab:lsc-scale}), 
%CAMERA READYwe shift from the LSC to the WiC setting as follow. First, we select only the annotated LSC instances containing contexts from different time periods. We then filtered out all the instances annotated by a single annotator\footnote{Different instances were annotated by varying numbers of annotators} and all the instances that are associated with an average score, $s$, such that $1.5 < s < 3.5$, which represents ambiguous cases even for humans. Finally, we binarized the LSC annotations by converting each $s \leq 1.5$ to \textit{False} (i.e. different meanings) and each $s \geq 3.5$ to \textit{True} (i.e., same meaning). 
%CAMERA READY: remove the line below
we only binarized the human annotations\footnote{We will report further details in Appendix after acceptance}.

Similar to TempoWiC, we randomly sample a limited number of instances to create trial, training, and test sets. Table~\ref{tab:datasets} shows the number of positive and negative examples for each set.


%\begin{table}[!ht]
%\centering
%\resizebox{0.45\columnwidth}{!}{%
%\begin{tabular}{lcl}
%\multirow{4}{*}{$\Bigg\uparrow$} & 4: & Identical         \\
%                            & 3: & Closely related   \\
%                            & 2: & Distantly related \\
%                            & 1: & Unrelated        
%\end{tabular}}
%\caption{The DURel relatedness scale used in~\citealp{schlechtweg2020semeval,schlechtweg2018diachronic}}
%\label{tab:lsc-scale}
%\end{table}

\section{Experimental setup}
In the following, we present our research questions (RQs) and the various setups we consider in our work. In our experiments, we evaluate the performance of ChatGPT 3.5 over the TempoWiC and HistoWiC test sets using both the official OpenAI API (ChatGTP API)\footnote{version 0.27.8} and web interface (ChatGPT Web)\footnote{the August 3 Version}. In particular, among the ChatGPT 3.5 models available through the API, we assess the performance of \verb|gpt-3.5-turbo|. Following~\citealp{loureiro2022tempowic}, we employ Macro-F1 for multiclass classification problems as evaluation metric. 

\subsection{ChatGPT prompts} 
Current ChatGPT evaluations are typically performed manually~\cite{laskar2023systematic}. When automatic evaluations are performed, they are typically followed by a manual post-processing procedure~\cite{KOCON2023ChatGPT}. As manual evaluation and processing may be biased due to answer interpretation, we address the following research question:\\

\textbf{RQ1}: \textit{Can we evaluate ChatGPT in WiC tasks completely in an automatic way?}\\

Furthermore, as current evaluations generally rely on a zero-shot prompting strategy, we address the following research question:\\

\textbf{RQ2}: \textit{Can we enhance ChatGPT's performance in WiC tasks by leveraging its in-context learning capabilities?}%CAMERA READY\\

To address RQ1 and RQ2, we design a prompt template to explicitly instruct ChatGPT to answer following the WiC label format (i.e., \textit{True}, \textit{False})%CAMERA READY: remove footnote
\footnote{We will report our template in Appendix after acceptance}. We then use this template with different prompt strategies: 
\begin{compactitem}
    \item \textit{zero-shot prompting} (ZSp): ChatGPT is asked to address the WiC tasks (i.e. test sets) without any specific training, generating coherent responses based solely on its pre-existing knowledge.
    \item \textit{few-shot prompting} (FSp): since PFs have recently demonstrated \textit{in-context learning} capabilities without requiring any fine-tuning on task-specific data~\cite{Brown2020Language}, ChatGPT is presented with a limited number of input-output examples (i.e. trial sets) demonstrating how to perform the task. The goal is to leverage the provided examples to improve the model's task-specific performance.
    \item \textit{many-shot prompting} (MSp): similar to FSp, but with a greater number of input-output examples (i.e. train sets).
\end{compactitem}

%CAMERA READY
%We report our template in Table~\ref{tab:prompt-strategies}. 

\subsection{ChatGPT temperature}
The temperature is a hyper-parameter of ChatGPT that regulates its variability of responses to human queries. According to the OpenAI FAQ, the temperature parameter ranges from 0.0 to 2.0, where lower values makes outputs mostly deterministic, whereas higher values makes outputs more random\footnote{\url{platform.openai.com/docs/api-reference/chat}}. To counteract the non-determinism of ChatGPT, we focus only on TempoWiC and HistoWiC and consider the effect of temperature by conducting the same experiment multiple times with progressively increasing temperatures. This way, we want to answer the following research questions:\\

% - [Francesco]: do you like more the actual RQ or this one: Does ChatGPT demonstrate comparable effectiveness in detecting short-term changes in contemporary text compared to long-term changes in historical text?
%Nina: I prefer the above, can we fit it?
\textbf{RQ3}: \textit{Does ChatGPT demonstrate comparable effectiveness in detecting short-term changes in contemporary text compared to long-term changes in historical text?}\\%\textit{Is ChatGPT equally effective at detecting short-term changes in contemporary text and long-term changes in historical text?}\\

\textbf{RQ4}: \textit{Can we enhance ChatGPT's performance in WiC tasks by raising the ``creativity'' through the temperature value?}\\

To address RQ3 and RQ4, we evaluate ChatGPT in TempoWiC and HistoWiC by using eleven temperatures in the range [0.0, 2.0] with 0.2 increments\footnote{$\{0.0, 0.2, 0.4, 0.6, 0.8, 1.0, 1.2, 1.4, 1.6, 1.8, 2.0\}$}. 
For each temperature and prompting strategy, we perform two experiments and consider the average performance. %we can still analyze the trend of ChatGPT's performance across lower and higher intermediate temperatures.

\subsection{ChatGPT API v ChatGPT Web}
Current evaluations typically prompt ChatGPT through the web interface instead of the official OpenAI API. This preference is due to the cost-free accessibility to the web interface and the fact that the official API was introduced at a later stage. However, we argue that that there are differences in using ChatGPT through the web interface (ChatGPT Web) compared to using the official API (ChatGPT API). As a matter of fact, although it is possible to test ChatGPT API with varying temperature, performing the same evaluation on ChatGPT Web is not feasible, as the temperature value cannot be controlled beyond being unknown. In contrast, while ChatGPT API allows a limited message history, ChatGPT Web seems to handle unlimited message history.

We compare the performance of ChatGPT API and Web to address the following research question:\\

\textbf{RQ5}: \textit{Does ChatGPT API demonstrate comparable performance to ChatGPT Web in solving WiC tasks?}\\

Testing ChatGPT API with the MSp strategy would be equivalent to testing it with the FSp strategy due to the limited message history. Thus, we evaluate ChatGPT Web with MSp  aiming to address the following research question:\\

\textbf{RQ6}: \textit{Can we enhance ChatGPT's performance in WiC tasks by providing it with a larger number of in-context examples?}\\

To address this research questions, we test both ChatGPT API and Web by using a single chat for each considered prompting strategy. Since testing ChatGPT API Web is extremely time demanding, we conduct one experiment for each prompting strategy. 

\subsection{ChatGPT v BERT}
The understanding capability of ChatGPT has been prompting the belief that ChatGPT is a \textit{jack of all trades} which makes previous technologies somewhat outdated. Drawing upon~\citealp{KOCON2023ChatGPT}, we believe that, when used for solving downstream task,  ChatGPT is a \textit{master of none} which work \textit{on a comparable level to the competitor but not outperforming any major SOTA solutions}.

By relying on multiple experiments on TempoWiC and HistoWiC, we aim to empirically assess the potential of ChatGPT for WiC and LSC tasks. In particular, we address the following research question:\\

\textbf{RQ7}: \textit{Does ChatGPT outperform BERT embeddings in detecting semantic changes?} \\

To address RQ7, we evaluate \verb|bert-base-uncased| on TempoWiC and HistoWiC over different layers. Recent research has indeed exhibited higher results when utilizing earlier layers rather than the final layers for solving downstream tasks~\cite{ma2019universal,coenen2019visualizing}. 
%CAMERA READY: periti2023time,liang2023named
For each layer, we extract the word embedding for a specific target word $w$ in the context $c_1$ and $c_2$. Since the focus of our evaluation is on ChatGPT, we do not fine-tune BERT and simply use the similarity between the embeddings of $w$ in the context $c_1$ and $c_2$. In particular, we follow~\citealp{pilehvar2019wic} and train a threshold-based classifier using the cosine distance between the two embeddings of each pair in the train set. The training process consists of selecting the threshold that maximizes the performance on the train set. We train a distinct threshold-based classifier for each BERT layer and for each WiC task (i.e., TempoWiC and HistoWiC). Then, in our evaluation, we apply these classifiers to evaluate BERT over the TempoWiC and HistoWiC test sets. \\

Finally, we address the following research question:\\

\textbf{RQ8}: \textit{Can we rely on the pre-trained knowledge of ChatGPT to automatically solve the LSC task?}\\

Since ChatGPT has demonstrated awareness of historical lexical semantic changes when manually asked about the lexical semantic changes of some words (e.g., \textit{plane}), our goal with RQ8 is to automatically test ChatGPT's pre-trained knowledge of historical semantic changes covered in the English LSC benchmark. We address this research question by relying on the LSC ranking task as defined in~\citealp{schlechtweg2018diachronic}. Thus, we specifically ask ChatGPT to rank the set of 37 target words in the English LSC benchmark according to their degree of LSC between two time periods, T1 (i.e., 1810--1860) and T2 (i.e., 1960--2010). For each temperature, we repeat the same experiment ten times, totaling 110 experiments\footnote{We will report our template in Appendix after acceptance}. %CAMERA READY: remove footnote
Then, for each temperature, we evaluate ChatGPT's performance by computing the Spearman correlation over gold scores derived from human annotation and the average ChatGPT score for each target. 

\section{Experimental results}
In this section, we report the results of our experiments, while discussing the answer of each research question\footnote{We provide all our data, code, and results after acceptance}.%CAMERA READY\\
%CAMERA READY
%{We provide all our data, code, and results at \url{https://github.com/FrancescoPeriti/LChange23}}.

\paragraph{RQ1:} %CAMERA READY\textit{Can we evaluate ChatGPT in WiC tasks completely in an automatic way?}\\

We observe that ChatGPT consistently respond following our template in nearly all cases, thereby allowing us to evaluate its answers completely without human intervention. As a general remark for ChatGPT API, we notice that the higher the temperature, the larger the tendency for deviations from the expected response format (see Figure~\ref{fig:wfa}). 
%\footnote{We will report the number of deviations in Appendix after acceptance}. 
ChatGPT Web answered with a wrong format only once.
%CAMERA READY
%(see Appendix~\ref{app:failure}). 
To ensure impartiality, we classified the few ChatGPT responses that do not adhere to the required format as incorrect answers. %CAMERA READY\\

\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{imgs/wfa.png}
\caption{Average number of Wrongly Formatted Answers (WFAs) over the considered temperature values}%CAMERA READY: Average number of ChatGPT's Wrongly Formatted Answers (WFAs) over the considered temperature values
\label{fig:wfa}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{imgs/chatgptapi.png}
\caption{ChatGPT's performance (Macro-F1) as temperature increases}%CAMERA READY: ChatGPT API's performance (Macro-F1) for TempoWiC and HistoWiC tasks with varying temperature values and prompting strategies
\label{fig:api-temperature}
\end{figure}

\paragraph{RQ2:} %CAMERA READY\textit{Can we enhance ChatGPT's performance in WiC tasks by leveraging its in-context learning capabilities?} \\

Figure~\ref{fig:api-temperature} shows the rolling average of ChatGPT API's performance across different temperatures, prompting strategies, and WiC tasks. By using a window size of 4, we are able to consider 8 different experiments per temperature\footnote{Except for the first and last two temperatures} (for each temperature, we run two experiments). Figure~\ref{fig:web-prompt} shows ChatGPT Web's performance across different prompting strategies and WiC tasks.

Figure~\ref{fig:api-temperature} and~\ref{fig:web-prompt} demonstrate that ZSp consistently outperforms FSp on HistoWiC. On the contrary, FSp consistently outperforms ZSp on TempoWiC when ChatGPT API is used. This suggests that the in-context learning capability of ChatGPT is more limited for historical data. Instead, in Figure~\ref{fig:web-prompt}, ChatGPT Web's performance with ZSp outperforms the one obtained with FSp for both TempoWiC and HistoWiC, even though the discrepancy is smaller. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{imgs/chatgptweb.png}
\caption{ChatGPT's performance (Macro-F1). Temperature is unknown}%CAMERA READY: ChatGPT Web's performance (Macro-F1) for TempoWiC and HistoWiC tasks with varying prompting strategies. Temperature is unknown for ChatGPT Web
\label{fig:web-prompt}
\end{figure}

\paragraph{RQ3:} %%CAMERA READY\textit{Is ChatGPT equally effective at detecting short-term changes in contemporary text and long-term changes in historical text?}\\

\begin{table}[!ht]
\centering
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{cc}
 & \textbf{Macro-F1} \\ \hline
 \citealp{chen2022using} & .770 \\
\citealp{loureiro2022tempowic} & .703 \\
%\citealp{loureiro2022tempowic} & .670 \\%CAMERA READY
%\citealp{lyu2022mllabs} & .625 \\%CAMERA READY
\textit{ChatGPT API} & .689 \\
\textit{ChatGPT Web} & .580 \\
\textit{BERT} & .743 \\
\end{tabular}%
}
\caption{Macro-F1 scores obtained by SOTA systems, ChatGPT (best score), and BERT (last layer)}%CAMERA READY: Comparison of (Macro-F1) scores obtained by SOTA systems on the full TempoWiC dataset and scores obtained on our TempoWiC subset using the ChatGPT API, ChatGPT Web, and BERT. For ChatGPT API and Web, we report the best score obtained in our experiments. For BERT, we report the score obtained using the last layer
\label{tab:sota-tempowic}
\end{table}

Figure~\ref{fig:api-temperature} and~\ref{fig:web-prompt} demonstrate that that ChatGPT's performance on TempoWiC is consistently lower compared to its performance on HistoWiC. In particular, we observe that ChatGPT's performance ranges from .551 to .689 on TempoWiC and from .552 to .765 on HistoWiC\footnote{We will report all our results in Appendix after acceptance}. %CAMERA READY: remove footnote. 
This suggest that ChatGPT is significantly more effective in long-term change detection than in short-term change detection. We believe that this might involve word meanings that were not explicitly covered during training, potentially aiding ChatGPT in detecting anomalies from the usual patterns. We will further investigate this aspect in our future research. % - [Francesco]: is this last sentence ok?

For the sake of comparison, we report SOTA performance in Table~\ref{tab:sota-tempowic}.

\paragraph{RQ4:} %%CAMERA READY\textit{Can we enhance ChatGPT's performance in WiC tasks by raising the ``creativity'' through the temperature value?}\\

Figure~\ref{fig:api-temperature} shows that, on average, higher performance is associated with lower temperatures for both TempoWiC and HistoWiC, with accuracy decreasing as temperature values increase. Thus, we argue that high temperatures do not facilitate ChatGPT in solving WiC tasks or identifying semantic changes effectively.%CAMERA READY\\

\paragraph{RQ5:} %%CAMERA READY\textit{Does ChatGPT API demonstrate comparable performance to ChatGPT Web in solving WiC tasks?}\\

ChatGPT Web results are presented in Table~\ref{tab:web}, along with the average performance we obtained through the ChatGPT API across temperature values ranging from 0.0 to 1.0 (API 0-1), from 1.0 to 2.0 (API 1-2), and from 0.0 to 2.0 (API 0-2). Similar to ChatGPT API, the performance of ChatGPT Web is higher for HistoWiC than for TempoWiC. In addition, our evaluation indicates that ChatGPT Web employs a moderate temperature setting, as we obtained consistent results when using a moderate temperature setting through ChatGPT API. This suggests that, for solving downstream task like WiC, the ChatGPT API should be preferred. This also suggests that the current SOTA evaluations may achieve higher results if the official API were used instead of the web interface.%CAMERA READY\\  

\begin{table}[!ht]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
 & \multicolumn{4}{c}{\textbf{TempoWiC}} & \multicolumn{4}{c}{\textbf{HistoWiC}} \\ \cline{2-9} 
\multicolumn{1}{c|}{} & \textit{API} & \textit{API} & \textit{API} & \multicolumn{1}{c|}{\textit{web}} & \textit{API} & \textit{API} & \textit{API} & \multicolumn{1}{c|}{\textit{web}} \\
\multicolumn{1}{c|}{Temp.} & 0 - 1 & 1 - 2 & 0 - 2 & \multicolumn{1}{c|}{-} & 0 - 1 & 1 - 2 & 0 - 2 & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{c|}{ZSp} & .609 & .589 & .600 & \multicolumn{1}{c|}{.580} & .713 & .665 & .688 & \multicolumn{1}{c|}{.686} \\
\multicolumn{1}{c|}{FSp} & .636 & .606 & .622 & \multicolumn{1}{c|}{.569} & .693 & .626 & .657 & \multicolumn{1}{c|}{.674} \\
\multicolumn{1}{c|}{MSp} & - & - & - & \multicolumn{1}{c|}{.500} & - & - & - & \multicolumn{1}{c|}{.565} \\ \hline
\multicolumn{1}{c|}{\textbf{all}} & .622 & .598 & .611 & \multicolumn{1}{c|}{.550} & .703 & .645 & .672 & \multicolumn{1}{c|}{.642}\\ \cline{2-9} 
\end{tabular}%
}
\caption{Comparison of ChatGPT API and ChatGPT Web performance (Macro-F1)} %CAMERA READY: Comparison of ChatGPT Performance (Macro-F1) for TempoWiC and HistoWiC tasks using ChatGPT API and ChatGPT Web. We consider the average scores obtained over various temperatures as ChatGPT API values
\label{tab:web}
\end{table}

\paragraph{RQ6:} %%CAMERA READY\textit{Can we enhance ChatGPT's performance in WiC tasks by providing it with a larger number of in-context examples?}\\

As shown in Figure\ref{fig:web-prompt}, as the number of example messages increases (from ZSp to MSp), the performance of ChatGPT Web decreases. This suggests that improving the performance of ChatGPT requires a more complex training approach than simply providing a few input-output examples. Furthermore, it indicates that the influence of message history is extremely significant in shaping the quality of conversations with ChatGPT. Indeed, a limited message history proved to be beneficial for the evaluation of ChatGPT API through FSp.%CAMERA READY\\

\paragraph{RQ7:} %%CAMERA READY\textit{Does ChatGPT outperform BERT embeddings in detecting semantic changes?} \\

Figure~\ref{fig:bert-layers} shows Macro-F1 scores obtained on TempoWiC and HistoWiC over the 12 BERT layers. When considering the final layer, which is conventionally adopted in downstream tasks, BERT obtains Macro-F1 scores of .750 and .743 for TempoWiC and HistoWiC, respectively. % CAMERA READY: Similar to~\citealp{periti2023time}, 
BERT performs best on HistoWiC when embeddings extracted from middle layers are considered. Instead, BERT performs best on TempoWiC when embeddings extracted from last layers are considered. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{imgs/layers.png}
\caption{Comparison of BERT Performance (Macro-F1) for TempoWiC and HistoWiC tasks across layers}
\label{fig:bert-layers}
\end{figure}

We compare the performance of ChatGPT and BERT across their respective worst to best scenarios by sorting the Macro-F1 scores obtained by BERT and ChatGPT in ascending order (bottom x-axis). For ChatGPT, we consider the results obtained through FSp and ZSp prompting for TempoWiC and HistoWiC, respectively. As shown in Figure~\ref{fig:gptvbert}, even when considering the best setting, ChatGPT does not outperform the Macro-F1 score obtained by using the last layer of BERT, marked with a black circle. However, although it exhibits lower performance, ChatGPT is still comparable to BERT results on HistoWiC when the last embeddings extracted from the last layer of BERT are used.

\begin{figure}[!t]
\centering
\includegraphics[width=0.6\columnwidth]{imgs/gptvbert-nolabel.png}
\caption{ChatGPT v BERT (Macro-F1). Performance are sorted in ascending order regardless of temperatures and layers. A black circle denotes the use of the last layer of BERT}%CAMERA READY: Comparison of BERT and ChatGPT performance (Macro-F1). Performance are sorted in ascending order regardless of temperatures and layers. For sake of comparison, we marked with a black circle the performance of BERT when the last layer is used for embedding extraction
\label{fig:gptvbert}
\end{figure}

Since our goal is to evaluate the potential of ChatGPT for recognizing lexical semantic changes, we analyze the True Negative Rate and False Negative Rate scores as \textit{negative} examples represents semantic change in TempoWiC and HistoWiC datasets. As shown in Figure~\ref{fig:tnrfnr}, regardless of the temperature and layer considered, ChatGPT fall short in recognizing semantic change for both TempoWiC and HistoWiC compared to BERT. However, it produces less False Negative than BERT for TempoWiC.\\

\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{imgs/tnrfnr.png}
\caption{True Negative Rate v False Negative Rate. Crosses and dots represents ChatGPT and BERT experiment respectively}%CAMERA READY: True Negative Rate v False Negative Rate using ChatGPT and BERT. Each cross represents a ChatGPT experiment on TempoWiC and HistoWiC. Each dot represents the use of a specific layer of BERT on TempoWiC and HistoWiC
\label{fig:tnrfnr}
\end{figure}

\paragraph{RQ8:} %%CAMERA READY\textit{Can we rely on the pre-trained knowledge of ChatGPT to automatically solve the LSC task?}\\

In our experiment, ChatGPT achieves low Spearman’s correlation coefficients for each temperature when asked to rank the target word of the LSC English benchmark by degree of lexical semantic change. Higher correlations were achieved by using low temperatures rather than high ones.
Table~\ref{tab:LSC} shows the ChatGPT correlation for the temperature 0. For the sake of comparison, we report correlations obtained by BERT-based systems that leverage pre-trained models. Note that, when BERT is fine-tuned, it generally achieves even higher correlation scores (see survey by~\citealp{montanelli2023survey}).

\begin{table}[!ht]
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{cc}
 & \textbf{Spearman’s correlation} \\ \hline
\citealp{laicher2021explaining} & .573 \\
\citealp{periti2022done} & .514 \\
%\citealp{rother2020cmce} & .512 \\ %CAMERA READY
\textit{ChatGPT API} & .251
\end{tabular}%
}
\caption{SOTA BERT-base systems v ChatGPT (temperature=0) - LSC comparison}
\label{tab:LSC}%CAMERA READY: Comparison of correlation obtained by SOTA BERT-based systems and correlation obtained by ChatGPT with temperature set to 0
\end{table}

As shown in Table~\ref{tab:LSC}, the BERT-based system largely outperforms ChatGPT, suggesting that ChatGPT is not well-adapted for use in solving LSC downstream tasks for now.

\subsection{BERT for Semantic Change Detection}
There are notable differences between the Macro-F1 for TempoWiC and HistoWiC in terms of how the results increase and decrease across layers (see Figure~\ref{fig:bert-layers}). For TempoWiC the results increase until the 8th layer, after which they remain almost stable. Conversely, for HistoWiC the BERT performance rapidly increases until the 5th layer, after which it linearly decreases until the 12th layer. As for Tempo WiC, we hypothesize that BERT is already aware of the set of word meanings considered for evaluation, as it was pre-trained on modern and contemporary texts. As for HistoWiC, we hypothesize that BERT is not completely aware of the set of word meanings considered for evaluation. This way, word representations adopted for the historical context of HistoWiC\footnote{1810 - 1860, as referenced in~\cite{schlechtweg2020semeval}} might be relatively tuned. Thus, using medium embedding layers could prove beneficial in detecting semantic changes, as these layers are less affected by contextualization~\cite{ethayarajh2019contextual}. In other words, for HistoWiC, we hypothesize that the performance diminishes in the later layers due to the increasing contextualization of the medium and final embedding layers, which %hinders 
reduces the presence of noise in untuned word representations. This prompts us to question the appropriateness of utilizing the last embedding layers for recognizing historical lexical semantic change detection. Addressing this query is a focus of our future research.

\section{Conclusion}
In this study, we empirically investigate the capability of ChatGPT in detecting \textit{semantic change}. We consider the TempoWiC benchmark for assessing ChatGPT's ability in detecting short-term semantic changes and introduce a novel benchmark, named HistoWiC, for assessing ChatGPT in recognizing long-term changes. Our experiments demonstrate that ChatGPT achieves comparable performance to BERT (although slightly lower) in detecting long-term changes but performs significantly worse in recognizing short-term changes. We find that BERT's contextualized embeddings consistently provide a more effective and robust solution for capturing both short and long-term changes in word meanings.

The discrepancy in ChatGPT's performance between TempoWiC and HistoWiC leads to two potential interpretations: i) HistoWiC might involve word meanings not explicitly covered during training, potentially aiding ChatGPT in detecting anomalies from the usual patterns; ii) TempoWiC involves patterns typical of Twitter, such as abbreviations, mentions, or tags, which may render it a more challenging task compared to HistoWiC.

In light of our findings, we argue that \textit{ChatGPT might be the hero the world deserves but not the one it needs right now}, in particular for computationally modeling meaning over time and by extension, 
for the study of semantic change.

\section*{Limitations}
Similar to all the research on ChatGPT~\cite{laskar2023systematic, KOCON2023ChatGPT, zhong2023chatgpt}, our work has a significant limitation that we cannot address: our ChatGPT results are not entirely reproducible, as ChatGPT is inherently non-deterministic. In addition, similar to~\citealp{zhong2023chatgpt,jiao2023chatgpt}, due to time and economic limits of testing ChatGPT, our evaluation is executed on a subset of the TempoWiC and HistoWiC dataset. %Furthermore, due to time constraints, we conducted only a single experiment for each prompting strategy when considering ChatGPT by using the web interface. A more convincing approach would involve testing ChatGPT on a larger sample size and conducting multiple rounds of experiments for each temperature and prompt strategy. In future work, we aspire to not only evaluate ChatGPT on a broader range of examples but also to conduct more in-depth analysis and discussion across similar outputs at different temperatures.

In our study, we utilized ChatGPT 3.5. It is worth noting that this choice could be considered a limitation, given the recent release of ChatGPT 4. Nonetheless, we opted for ChatGPT 3.5 based on the guidance provided in the OpenAI documentation\footnote{\url{https://platform.openai.com/docs/guides/gpt/which-model-should-i-use}}. We acknowledge, however, that OpenAI continues to train and release new models, which could potentially impact the reproducibility of our results.

One of the many features of ChatGPT is its ability to incorporate the history of preceding messages within a conversation while responding to new input prompts. However, there remain several unanswered questions regarding how this history influences the model's answers. This holds true even for the zero-shot prompting strategy, where a general setting is lacking. Multiple prompts can be provided as part of the same chat or across different chats. For simplicity, we assigned only one chat for each ZSp experiment. Nonetheless, we intend to use different chats in our future work to examine and investigate the effect of the message history.

Finally, as highlighted by~\citealp{laskar2023systematic}, since the instruction-tuning datasets of OpenAI models are unknown (that is, not open-source), the datasets used for evaluation may or may not exist in the instruction-tuning training data of OpenAI. However, despite these limitations, we argue that our work is still significant, as it may prompt new discussions on the use of PFMs such as BERT and ChatGPT, as well as dispel the expanding belief that ChatGPT makes BERT an outdated technology.

% CAMERA READY
%\section*{Acknowledgements}
%This work has in part been funded by the project Towards Computational Lexical Semantic Change Detection supported by the Swedish Research Council (2019–2022; contract 2018-01184), and in part by the research program Change is Key! supported by Riksbankens Jubileumsfond (under reference number M21-0021).

% CAMERA READY
%\section{Optional Supplementary Materials}
%Appendices or supplementary material (software and data) will be allowed ONLY in the final, camera-ready version, but not during submission, as papers should be reviewed without the need to refer to any supplementary materials.

%Each \textbf{camera ready} submission can be accompanied by an appendix usually being included in a main PDF paper file, one \texttt{.tgz} or \texttt{.zip} archive containing software, and one \texttt{.tgz} or \texttt{.zip} archive containing data.

%We encourage the submission of these supplementary materials to improve the reproducibility of results and to enable authors to provide additional information that does not fit in the paper. For example, preprocessing decisions, model parameters, feature templates, lengthy proofs or derivations, pseudocode, sample system inputs/outputs, and other details necessary for the exact replication of the work described in the paper can be put into the appendix. However, the paper submissions must remain fully self-contained, as these supplementary materials are optional, and reviewers are not even asked to review or download them. If the pseudo-code or derivations, or model specifications are an essential part of the contribution, or if they are important for the reviewers to assess the technical correctness of the work, they should be a part of the main paper and not appear in the appendix. Supplementary materials need to be fully anonymized to preserve the double-blind reviewing policy.

%\subsection{Appendices}

%Appendices are material that can be read and include lemmas, formulas, proofs, and tables that are not critical to the reading and understanding of the paper, as in \href{https://acl-org.github.io/ACLPUB/formatting.html#appendices}{*ACLPUB}. It is  highly recommended that the appendices should come after the references; the main text and appendices should be contained in a `single' manuscript file, without being separately maintained. Letter them in sequence and provide an informative title: \textit{Appendix A. Title of Appendix}


%\subsection{Extra space for ethical considerations and limitations}

%Please note that extra space is allowed after the 8th page (4th page for short papers) for an ethics/broader impact statement and a discussion of limitations. At submission time, if you need extra space for these sections, it should be placed after the conclusion so that it is possible to rapidly check that the rest of the paper still fits in 8 pages (4 pages for short papers). Ethical considerations sections, limitations, acknowledgments, and references do not count against these limits. For camera-ready versions, nine pages of content will be allowed for long (5 for short) papers.


%

==> main_new.tex <==
%TODO: Addressing the identified weaknesses
%REVIEW 1 --
%Scientific relevance: We would like to highlight the significance of our work in raising awareness about the limited understanding of models like ChatGPT, despite their popularity and widespread enthusiasm. Our intention is to underscore the challenges researchers should be aware of when utilizing such models and to emphasize the importance of our findings in the context of Semantic Change Detection. We would like to draw attention to the ongoing research efforts, including a recent work [1] that underscores the increasing capacities of large language models in humanities and social sciences. We believe that this work aligns with our objective. For instance, our work holds relevance as it investigates the suitability of ChatGPT in detecting semantic changes and assisting human annotators for developing new WiC and LSC datasets, a critical aspect given the limited availability of datasets covering more than two time periods. We will incorporate relevant information from the referenced work [1] to further emphasize the importance of our research in the broader context of utilizing LLMs for data analytics in the humanities and social sciences.

%Comparison of Different Models: We appreciate the feedback on the conceptual differences between BERT and ChatGPT. In our revised version for the camera-ready, we will clarify the choices made in our experimental setup. Regarding the choice of ChatGPT for our study, we want to emphasize that our decision was driven by recent comparative work on the use of ChatGPT for various NLP tasks (e.g. [2], [3]). We are aware of alternative open-source solutions, such as LLAMA, but i) based on the current literature, we found ChatGPT to be superior in performance; ii) open-source solutions requires expensive GPUs for usage, making it less accessible for researchers with limited resources.

%Additions for Camera-Ready Version: In the camera-ready version, with an additional page, we will provide an example of LSC, more details on the datasets, including information about word embeddings for subtokens (we averaged them), and we will explicitly mention the task for which earlier layers exhibited better performance (we have already mentioned the corresponding references in our paper). We will also add this very recent work showing better performance for WiC by using early layers [4].

%REVIEW 2 --
%Model Choice and Comparison: We chose BERT as it represents the State-of-the-Art (SOTA) in LSC[1]. In contrast, XLM-R did not exhibit superior performance compared to BERT[2,3]. We opted for ChatGPT due to its increasing popularity and ease of testing compared to resource-intensive open-source models like LLAMA. Unfortunately, our current alternative involves paying OpenAI for using GPT models or investing in expensive and substantial GPU resources. We will emphasize that our primary focus was not to make a comprehensive comparison for all (L)LM and chat-like models, but rather to engage the canonical/common one, and specifically target the scenario of Semantic Change Detection

%Evaluation Practices and Related Work: Current evaluations have predominantly focused on assessing the model's overall capabilities rather than its performance on specific tasks. We delineate the primary issues in these evaluations, such as overlooked non-determinism, reliance on a single zero-shot prompt, and the use of the web interface. In our paper, we refer to related evaluations that support our perspective and discuss the implications of such practices. Furthermore, we challenge the current suboptimal performance of ChatGPT in the WiC task, with accuracy rates of 62% and 64% as reported in [4] and [5] respectively. While it is true that recent evaluations may use the OpenAI API, we explicitly cited papers discussing manual evaluations due to the unavailability of the API in the past year. We highlighted a significant evaluation campaign mentioned in our paper, emphasizing the continued use of manual evaluations even in recent research efforts [4]. We will ensure our camera ready version reflects the dynamic nature of evaluation practices

%Cost and rate limitations: We appreciate your observation regarding the emphasis on the cost argument. We will include a detailed cost estimate in our camera-ready paper, taking into account both financial implications and processing time. Furthermore, with regard to hourly token processing limits, we recognize the dynamic nature of model documentation. In our camera-ready version, we will provide the following links for reference: i) Pricing: https://openai.com/pricing; ii) Rate limits: https://platform.openai.com/docs/guides/rate-limits?context=tier-free

%Many-shot vs Few-shot: We justify the choice of many-shot by drawing on insights from few-shot learning literature. In few-shot scenarios, models may risk overfitting due to the limited training examples. In contrast, many-shot prompting allows for a more comprehensive exploration of the gold data distribution, promoting the learning of a well-generalized model [6]. We will reference other works supporting the effectiveness of a larger number of shots for improved model generalization.

%Few-shots vs Zero-shot: While we acknowledge the limited scope of our few-shots vs zero-shot comparison, we emphasize that our goal is to provide a straightforward and reasonable comparison assessment of ChatGPT for detecting semantic changes in an automatic way and by user interactions. Other detailed comparisons extend beyond the focus of our paper.

%Transferability of results and impact of our work: We strongly believe that our results offer valuable insights for the LSC community, particularly in the context of machine-assisted annotation and benchmark development. We will elaborate on these points to underscore the relevance and impact of our findings. In addition, while acknowledging the capabilities of ChatGPT, we express concerns regarding the current state of evaluations (see Scientific Relevance in Review 3)

\section{Introduction}
Lexical semantic change is the linguistic phenomenon that denotes words changing their meanings over time~\cite{geeraerts2024lexical,bloomfield1933language}. These changes can be radical, like how the word \texttt{gay} changed its meaning completely from \texttt{cheerful} to \texttt{homosexual}, but they can also be more subtle. An example can be observed in the Italian words \texttt{presidente} and \texttt{presidentessa} that changed from meaning \texttt{male president} and \texttt{wife of the president} to encompass broader meanings of \texttt{president of either sex} and \texttt{female president}, respectively\footnote{This transformation was prompted by 20th-century movements that advocated for women's rights to exercise professional roles with full legal and economic equality, while criticizing the derivation of female professional names from their male counterparts. \url{https://accademiadellacrusca.it/it/consulenza/la-} \url{presidente-dellaccademia-della-crusca-ancora-sul-} \url{femminile-professionale/250}}. These kind of changes are crucial to our understanding of historical texts, and the phenomena included in these text. But they are equally relevant when studying out-of-domain texts, that is, texts in which the language differs from the general language, like medical and legal texts or in radical groups. The capability to computationally gain a nuanced grasp of semantic \textit{variation} between groups and genre, and semantic \textit{change} across time  is important. It allows us to study languages, cultures, and societies through digitized text. It opens up a range of research applications from linguistic research and historical studies to social sciences. Computational approaches to semantic change are thus tools with immense potential for a range of research fields~\cite{tahmasebi2023computational,Tahmasebi2021}. Not only can they broaden the field of historical linguistics and simplify lexicography, but they can also be fruitfully applied in any text-based research %field 
(e.g., ~\citealp{paccosi2023sensibility,menini2022multilingual}). 

These computational approaches include both the computational representation of word meaning, and the detection of change~\cite{montanelli2023survey,nina2021survey,kutuzov2018diachronic}. Critically, the study of semantic change can also be used to evaluate the true capacity for generalization of large language models, for it serves as a litmus test of their ability to handle text under unique out-of-distribution (OOD) conditions. For example, a modern, ``gender-inclusive'' model trained on contemporary text might misinterpret the Italian expression \texttt{il presidente e la presidentessa} in historical documents, interpreting it as two presidents (one male and one female) rather than as \textit{the president and his wife}.

The recent introduction of Transformer-based~\cite{Vaswani2017attention} language models (LMs) has led to significant advances in Natural Language Processing (NLP). These advances are exemplified in Pretrained Foundation Models like BERT~\cite{devlin2019bert} and (Chat)GPT~\cite{Brown2020Language}, which ``\textit{are regarded as the foundation for various downstream tasks}''~\cite{zhou2023comprehensive}.  BERT has experienced a surge in popularity over the last few years, and the family of BERT models has repeatedly provided state-of-the-art (SOTA) results for computational modeling of semantic change~\cite{cassotti2023xl,periti2023studying}. However, research focus is now shifting toward ChatGPT due to its impressive ability to generate fluent and high-quality responses to human queries, making it the fastest-growing AI tool. Several recent research studies have assessed the language capabilities of ChatGPT by using a wide range of prompts to solve popular NLP tasks~\cite{laskar2023systematic,KOCON2023ChatGPT}. However, current evaluations generally (a) overlook the fact that the output of ChatGPT is nondeterministic,\footnote{\url{platform.openai.com/docs/guides/gpt/faq}} and (b) rely only on contemporary and synchronic text, (c) consider the web interface,\footnote{\url{chat.openai.com}} which is the Chat version of the foundational GPT model.

As a result, these evaluations provide valuable insights into the generative, pragmatic, and semantic capabilities of ChatGPT~\cite{KOCON2023ChatGPT}, but fall short when %it comes to 
assessing its potential to solve NLP tasks and specifically to handle on historical and diachronic text, which constitutes a unique scenario for testing models’ ability to generalize. 

%Nina: I added this but I'm a bit unsure about it. 
%Francesco: We are using to much space for the intro. I don't think there is a need to emphasize more
%In this paper, we evaluate ChatGPT in comparison to BERT in this unique scenario and test the models' ability to generalize to historical text and a very challenging research task. Because of the costs associated with using a model like ChatGPT, we believe that our work can help other researchers evaluate the model for their semantic change task. 


%@Francesco, here would be a good place to put in some aspects of: Our experiments show that ... and then some example on tips and tricks on how to use GPT (and to be a bit cautious because it is not hte same as CHatGPT (with hisotry of prompts etc). 

\paragraph{Evaluation purpose.}
In this paper, we propose to evaluate the capability of ChatGPT to recognize (lexical) \textit{semantic change}, often also referred to as \textit{semantic shift}. Although the Lexical Semantic Change (LSC) evaluation task has recently been proposed in NLP~\cite{schlechtweg2020semeval}, its setup is not suitable for evaluating a model like ChatGPT due to the limited size of ChatGPT's prompts and answers, as well as accessibility limitations such as an hourly character limit and economic constraints. LSC involves identifying words that change meanings over time in a diachronic corpus. Typically, this task is approached by considering all usages of a word across two or more time periods. Contextual embeddings for the target word are gathered from each sentence for the different time periods. These are then compared either pairwise (for average-pairwise comparisons) or averaged per time period and then compared (using a prototype distance)~\cite{giulianelli-kutuzov?}.  Benchmarks exist on which the task can be evaluated on a range of languages, including the SemEval-2020 Task 1 \cite{schlechtweg2020semeval}. However, because these datasets can consist of several thousand sentences for each target word, they are too large to fit into a ChatGPT prompt (and answer). The accessibility limitations such as an hourly character limit and economic constraints are also important limitations. 

In light of this, we chose to evaluate the potential of ChatGPT through the Word-in-Context (WiC) task, which has recently demonstrated a robust connection with LSC~\cite{cassotti2023xl,arefyev2021deep} via the subtask of measuring pairwise distance. In particular, we consider two diachronic extensions of the original WiC setting, namely \textit{temporal} WiC (TempoWiC) and \textit{historical} WiC (HistoWiC). Our goal is to determine whether a word carries the same meaning in two different contexts stemming from different time periods.%Nina: are we not doing within time periods? 
If the meaning of the word is not the same across contexts, this either indicates that the word is used in two different meaning (existing polysemy), that it exemplify a semantic change. The word has hence gained a new sense that it did not previously had (or that it has lost). 

While TempoWiC has been designed to evaluate LMs ability to detect short-term changes in social media~\cite{loureiro2022tempowic}, HistoWiC is our adaptation of the SemEval-2020 LSC benchmark of historical text to a WiC task for evaluating LMs ability to detect long-term changes in historical corpora~\cite{schlechtweg2020semeval}. 

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{imgs/meme.png}
\caption{The title of this paper draws inspiration by the movie \textit{Batman v Superman: Dawn of Justice}. We leverage the analogy of ChatGPT and BERT, powerful and popular LMs, as two lexical superheroes often erroneously associated for solving similar problems. Our aim is to shed lights on the potential of ChatGPT and the, for semantic change detection, equally potent BERT model.}
\label{fig:meme}
\end{figure}

Considering the remarkable performance of contextualized BERT models in addressing WiC and LSC tasks~\cite{montanelli2023survey,periti2023time,periti2023studying}, we compare the performance of ChatGPT in TempoWiC and HistoWiC to those obtained using BERT. While BERT is specifically designed to understand the meaning of words in context, ChatGPT is designed to generate fluent and coherent text. In this paper we propose to use these two \textit{lexical superheros} (see Figure~\ref{fig:meme}), to illuminate the potential of ChatGPT and mark the dawn of a new era by empirically assessing whether ChatGPT makes the common approaches to WiC and LSC, which rely on similarities among BERT embeddings, outdated.

\textbf{We now need a new good ending sentence/paragraph for this subsection}


\section{Related work}
The significant attention garnered by ChatGPT has led to a large number of studies being published immediately after its release. Early studies focused mainly on exploring the benefits and risks associated with using ChatGPT in expert fields such as education~\cite{lund2023chatting}, medicine~\cite{ANTAKI2023100324}, or business~\cite{Shaji2023Review}. Evaluation studies are currently emerging for assessing ChatGPT's generative and linguistic  capabilities across a wide range of downstream tasks in both monolingual and multilingual setups~\cite{bang2023multitask,shen2023hugginggpt,lai2023chatgpt}.

Most evaluations involve a limited number of instances (e.g., 50) for each task considered~\cite{weissweiler2023counting,zhong2023chatgpt,alberts2023large,khalil2023chatgpt}. When the official API is used to query ChatGPT, this limit is imposed by the hourly token processing limit\footnote{\url{help.openai.com/en/articles/4936856-what-}\\\url{are-tokens-and-how-to-count-them}} and the associated costs.\footnote{\url{openai.com/pricing}} When the web interface is used instead of the API, the limit is due to the time-consuming process of interacting with ChatGPT that keeps humans in the loop. Furthermore, even systematic and comprehensive evaluations ~\cite{KOCON2023ChatGPT,laskar2023systematic} rely on repetition of a single experiment for each task. 

While individual experiments provide valuable insights into ChatGPT's capabilities, they fall short in assessing the potential of ChatGPT to solve specific tasks given its nondeterministic nature. Multiple experiments need to be conducted to validate its performance on each task. In addition, current  evaluations generally leverage tasks that overlook the temporal dimension of text, leaving a gap in our understanding of ChatGPT's ability to handle diachronic and historical text.

\paragraph{Our original contribution.}
Our evaluation of ChatGPT focuses on two diachronic extensions of the WiC task, namely TempoWiC and HistoWiC. Our aim is to assess the potential of ChatGPT for \textit{semantic change detection}. To the best of our knowledge, this paper is the first to investigate the application of ChatGPT for historical linguistic purposes. 

Thus far, the  use of ChatGPT for a conventional WiC task has been evaluated only by~\newcite{laskar2023systematic} and~\newcite{KOCON2023ChatGPT}, who reported low accuracy % of 62.1\% and 64.58\%, 
under a single setup. In this paper, we challenge their performance by considering diachronic text and the following setups, totaling 47 experiments each for TempoWiC and HistoWiC:
\begin{itemize}
    \item \textbf{ChatGPT prompts}. \ Like~\newcite{zhong2023chatgpt}, we evaluate ChatGPT using zero-shot and few-shot prompting strategies, while also exploring many-shot prompting. Our results demonstrate that zero-shot prompting is more effective on HistoWiC, while few-shot prompting is more effective on TempoWiC. 

    \item \textbf{ChatGPT temperature}. \ Like~\newcite{peng2023making,liu2023code}, we analyze how ChatGPT's performance varies according to its temperature hyperparameter, which controls the ``creativity'' or randomness of its answers. Our results indicate that ChatGPT used with low temperature values (i.e., less creativity) is better at handling WiC tasks. 
    
    \item \textbf{ChatGPT API v ChatGPT Web}. \ We empirically assess whether ChatGPT produces worse results through the OpenAI API compared to the web interface.\footnote{Discussions on this topic are currently very active, for example,~\url{community.openai.com/t/web-app-vs-api-}\\\url{results-web-app-is-great-api-is-pretty-awful/96238}} Our results demonstrate that using the official API for WiC tasks is better than using ChatGPT through the web interface, as has previously been done~\cite{laskar2023systematic,KOCON2023ChatGPT}. Furthermore, our findings suggest that the web interface automatically sets an intermediate temperature for ChatGPT.

    \item \textbf{ChatGPT v BERT}. \ Finally, like~\newcite{zhong2023chatgpt}, we compare the performances of ChatGPT and BERT. By leveraging the TempoWiC task and introducing the novel \textbf{HistoWiC} task, we shed light on the potential of both models and demonstrate the superiority of BERT in dealing with diachronic text and WiC tasks.
\end{itemize}

\section{Semantic Change Detection}
Our evaluation relies on two diachronic definitions of the conventional Word-in-Context (WiC) task~\cite{pilehvar2019wic}, namely TempoWiC and HistoWiC. WiC is framed as a binary classification problem, where each instance is associated with a target word $w$,  either a verb or a noun, for which two contexts, $c_1$ and $c_2$, are provided. The task is to identify whether the occurrences of $w$ in $c_1$ and $c_2$ correspond to the same meaning or not. Both TempoWiC and HistoWiC rely on the same definition of the task, while being specifically designed for semantic change detection in diachronic text.

\subsection{Temporal Word-in-Context}
NLP models struggle to cope with new content and trends. TempoWiC is designed as an evaluation benchmark to detect short-term semantic changes on social media, where the language is extremely dynamic.  It  uses tweets from different time periods as contexts $c_1$ and $c_2$.

Given the limits on testing ChatGPT, we followed~\newcite{zhong2023chatgpt,jiao2023chatgpt} and randomly sampled a subset of the original TempoWiC datasets. While the original TempoWiC framework provides trial, train, test, and dev sets, here we did not consider the dev set. Table~\ref{tab:datasets} shows the number of positive (i.e., same meaning) and negative (i.e., different meanings due to semantic change) examples we considered for each set.

\begin{table}[!ht]
\centering
\caption{Datasets used in our evaluation} 
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{ccccccc}
                                   & \multicolumn{3}{c}{\textbf{TempoWiC}}     & \multicolumn{3}{c}{\textbf{HistoWiC}}     \\ \cline{2-7} 
\multicolumn{1}{c|}{}              & Trial & Train & \multicolumn{1}{c|}{Test} & Trial & Train & \multicolumn{1}{c|}{Test} \\ \cline{2-7} 
\multicolumn{1}{c|}{\textit{True}} & 8     & 86    & \multicolumn{1}{c|}{73}   & 11    & 137   & \multicolumn{1}{c|}{79}   \\
\multicolumn{1}{c|}{\textit{False}} & 12 & 114 & \multicolumn{1}{c|}{127} & \textit{9} & 103 & \multicolumn{1}{c|}{61} \\ \cline{2-7} 
\multicolumn{1}{c|}{\textbf{Total}}  & 20    & 200   & \multicolumn{1}{c|}{200}  & 20    & 200   & \multicolumn{1}{c|}{140}  \\ \cline{2-7} 
\end{tabular}}
\label{tab:datasets}
\end{table}

\subsection{Historical Word-in-Context}
Given that NLP models struggle to cope with historical content and trends, we designed HistoWiC as a novel evaluation benchmark for detecting long-term semantic change in historical text, where language may vary across different epochs. HistoWiC sets the two contexts, $c_1$ and $c_2$, as sentences collected from the two English corpora of the SemEval-2020 LSC detection task ~\cite{schlechtweg2020semeval}. 

As with WiC, the annotation process for the LSC benchmark involved usage pair annotations where a target word is used in two different contexts. We directly used the annotated instances of LSC to develop HistoWiC. Since LSC instances were annotated  using the DURel framework and a four-point semantic-relatedness scale~\cite{schlechtweg2020semeval,schlechtweg2018diachronic}, we only binarized the human annotations (see Appendix~\ref{app:fromLSCtoHistoWiC}).

As with TempoWiC, we randomly sampled a limited number of instances to create trial, training, and test sets. Table~\ref{tab:datasets} shows the number of positive and negative examples for each set.

\section{Experimental setup}
In the following, we present our research questions (RQs) and the various setups we considered in our work. In our experiments, we evaluated the performance of ChatGPT 3.5 over the TempoWiC and HistoWiC test sets using both the official OpenAI API (ChatGTP API)\footnote{version 0.27.8.} and the web interface (ChatGPT Web).\footnote{The August 3 Version.} Of the ChatGPT 3.5 models available through the API, we assessed the performance of \verb|gpt-3.5-turbo|. Following~\newcite{loureiro2022tempowic}, we employed the Macro-F1 for multiclass classification problems as evaluation metric. 

\subsection{ChatGPT prompts} 
Current ChatGPT evaluations are typically performed manually~\cite{laskar2023systematic}. When automatic evaluations are performed, they are typically followed by a manual post-processing procedure~\cite{KOCON2023ChatGPT}. As manual evaluation and processing may be biased due to answer interpretation, we addressed the following research question:\\

\textbf{RQ1}: \textit{Can we evaluate ChatGPT in WiC tasks  in a completely automatic way?}\\

Furthermore, as current evaluations generally rely on a zero-shot prompting strategy, we addressed the following research question:\\

\textbf{RQ2}: \textit{Can we enhance ChatGPT's performance in WiC tasks by leveraging its in-context learning capabilities?} %%CAMERA READY: \\

To address RQ1 and RQ2, we designed a prompt template to explicitly instruct ChatGPT to answer in accordance with the WiC label format (i.e., \textit{True}, \textit{False}). We then used this template (see Appendix~\ref{app:WiCtemplate}) with different prompt strategies: 
\begin{compactitem}
    \item \textit{zero-shot prompting} (ZSp): ChatGPT was asked to address the WiC tasks (i.e., test sets) without any specific training, generating coherent responses based solely on its preexisting knowledge.
    \item \textit{few-shot prompting} (FSp): since PFMs have recently demonstrated \textit{in-context learning} capabilities without requiring any fine-tuning on task-specific data~\cite{Brown2020Language}, ChatGPT was presented with a limited number of input-output examples (i.e., trial sets) demonstrating how to perform the task. The goal was to leverage the provided examples to improve the model's task-specific performance.
    \item \textit{many-shot prompting} (MSp): similar to FSp, but with a greater number of input-output examples (i.e., training sets).
\end{compactitem}

\subsection{ChatGPT temperature}
The temperature is a hyperparameter of ChatGPT that regulates the variability of responses to human queries. According to the OpenAI FAQ, the temperature parameter ranges from 0.0 to 2.0, with lower values making outputs mostly deterministic and higher values making them more random.\footnote{\url{platform.openai.com/docs/api-reference/chat}} To counteract the nondeterminism of ChatGPT, we focused only on TempoWiC and HistoWiC and conducted the same experiment multiple times with progressively increasing temperatures. This approach enabled us to answer the following research questions:\\

\textbf{RQ3}: \textit{Does ChatGPT demonstrate comparable effectiveness in detecting short-term changes in contemporary text and long-term changes in historical text?}\\

\textbf{RQ4}: \textit{Can we enhance ChatGPT's performance in WiC tasks by raising the ``creativity'' using the temperature value?}\\

To address RQ3 and RQ4, we evaluated ChatGPT in TempoWiC and HistoWiC using eleven temperatures in the range [0.0, 2.0] with 0.2 increments.\footnote{$\{0.0, 0.2, 0.4, 0.6, 0.8, 1.0, 1.2, 1.4, 1.6, 1.8, 2.0\}$} 
For each temperature and prompting strategy, we performed two experiments and considered the average performance. 

\subsection{ChatGPT API v ChatGPT Web}
Current evaluations typically prompt ChatGPT through the web interface instead of the official OpenAI API. This preference exists because the web interface is free and predates the official API. However, there are differences between using ChatGPT through the web interface (ChatGPT Web) and  the official API (ChatGPT API). For example, the ChatGPT API can be set to test at varying temperatures, but the temperature value on ChatGPT Web cannot be controlled. However,  while the ChatGPT API allows a limited message history, ChatGPT Web seems to handle an unlimited message history (see Appendix~\ref{app:history}).

We used the following research question to compare the performance of ChatGPT API and Web:\\

\textbf{RQ5}: \textit{Does ChatGPT API demonstrate comparable performance to ChatGPT Web in solving WiC tasks?}\\

Testing ChatGPT API with the MSp strategy would be equivalent to testing it with the FSp strategy due to the limited message history. Thus, we evaluated ChatGPT Web with MSp,  aiming to address the following research question:\\

\textbf{RQ6}: \textit{Can we enhance ChatGPT's performance in WiC tasks by providing it with a larger number of in-context examples?}\\

To address these research questions, we tested both ChatGPT API and Web using a single chat for each prompting strategy considered. Since testing ChatGPT Web is extremely time-consuming, we conducted one experiment for each prompting strategy. 

\subsection{ChatGPT v BERT}
The ability of ChatGPT to understand has prompted the belief that ChatGPT is a \textit{jack of all trades} that makes previous technologies somewhat outdated. Drawing upon~\newcite{KOCON2023ChatGPT}, we believe that, when used for solving downstream tasks,  ChatGPT is a \textit{master of none. } It works on a comparable level to the competition, but does not outperform any major SOTA solutions.

By relying on multiple experiments on TempoWiC and HistoWiC, we aimed to empirically assess the potential of ChatGPT for WiC and LSC tasks. In particular, we addressed the following research question:\\

\textbf{RQ7}: \textit{Does ChatGPT outperform BERT embeddings in detecting semantic changes?} \\

To address RQ7, we evaluated \verb|bert-base-uncased| on TempoWiC and HistoWiC over different layers. Recent research has exhibited better results when utilizing earlier layers rather than the final layers for solving downstream tasks such as WiC~\cite{periti2023time,ma2019universal,coenen2019visualizing,liang2023named}. For each layer, we extracted the word embedding for a specific target word $w$ in the context $c_1$ and $c_2$. Since the focus of our evaluation was on ChatGPT, we did not fine-tune BERT and simply used the similarity between the embeddings of $w$ in the context $c_1$ and $c_2$. In particular, we followed~\newcite{pilehvar2019wic}, and trained a threshold-based classifier using the cosine distance between the two embeddings of each pair in the training set. The training process consisted of selecting the threshold that maximized the performance on the training set. We trained a distinct threshold-based classifier for each BERT layer and for each WiC task (i.e., TempoWiC and HistoWiC). Then, in our evaluation, we applied these classifiers to evaluate BERT over the TempoWiC and HistoWiC test sets. \\

Finally, we addressed the following research question:\\

\textbf{RQ8}: \textit{Can we rely on the pretrained knowledge of ChatGPT to automatically solve the LSC task?}\\

Since ChatGPT has demonstrated awareness of historical lexical semantic changes when manually asked about the lexical semantic changes of some words (e.g., \textit{plane}), our goal with RQ8 was to automatically test ChatGPT's pretrained knowledge of historical semantic changes covered in the English LSC benchmark. In addressing this research question we relied on the LSC ranking task as defined in~\newcite{schlechtweg2018diachronic}. Thus, we specifically asked ChatGPT to rank the set of 37 target words in the English LSC benchmark according to their degree of LSC between two time periods, T1 (1810--1860) and T2 (1960--2010). For each temperature, we repeated the same experiment ten times, totaling 110 experiments. Then, for each temperature, we evaluated ChatGPT's performance by computing the Spearman correlation using gold scores derived from human annotation and the average ChatGPT score for each target (see Appendix~\ref{app:LSCtemplate}). 

\section{Experimental results}
In this section, we report the results of our experiments, while discussing the findings in regard to each research question.\footnote{We provide all our data, code, and results at \url{https://github.com/FrancescoPeriti/ChatGPTvBERT}}

\paragraph{RQ1:} %CAMERA READY\textit{Can we evaluate ChatGPT in WiC tasks  in a completely automatic way?}\\

ChatGPT consistently followed our template in nearly all cases, thereby allowing us to evaluate its answers without human intervention. For ChatGPT API, however, we noticed that the higher the temperature, the larger the tendency for deviations from the expected response format (see Figure~\ref{fig:wfa}). ChatGPT Web only once answered with an incorrect format. To ensure impartiality, we classified the few ChatGPT responses that did not adhere to the required format as incorrect answers. %%CAMERA READY: \\

\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{imgs/wfa.png}
\caption{Average number of wrongly formatted answers (WFAs) over the  temperature values considered. Background lines correspond to each experiment.}
\label{fig:wfa}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{imgs/chatgptapi.png}
\caption{Performance of ChatGPT API (Macro-F1) as temperature increases.} 
%\caption{Performance of ChatGPT API (Macro-F1) for TempoWiC and HistoWiC tasks with varying temperature values and prompting strategies}.
\label{fig:api-temperature}
\end{figure}

\paragraph{RQ2:} %%CAMERA READY: \textit{Can we enhance ChatGPT's performance in WiC tasks by leveraging its in-context learning capabilities?} \\

Figure~\ref{fig:api-temperature} shows the rolling average of the performance  of ChatGPT API across different temperatures, prompting strategies, and WiC tasks. By using a window size of 4, we were able to consider 8 different experiments per temperature.\footnote{Except for the first and last two temperatures.} (for each temperature, we ran two experiments) Figure~\ref{fig:web-prompt} shows the performance of ChatGPT Web across different prompting strategies and WiC tasks.

Figure~\ref{fig:api-temperature} and~\ref{fig:web-prompt} show that ZSp consistently outperforms FSp on HistoWiC. By contrast, FSp consistently outperforms ZSp in TempoWiC when the ChatGPT API is used. This result suggests that the in-context learning capability of ChatGPT is more limited for historical data. In Figure~\ref{fig:web-prompt}, ChatGPT Web's performance with ZSp outperforms that obtained with FSp for both TempoWiC and HistoWiC, although the discrepancy is smaller. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{imgs/chatgptweb.png}
\caption{Performance of ChatGPT Web (Macro-F1). Temperature is unknown.} %\caption{Performance of ChatGPT Web  (Macro-F1) for TempoWiC and HistoWiC tasks with varying prompting strategies. Temperature is unknown for ChatGPT Web.}
\label{fig:web-prompt}
\end{figure}

\paragraph{RQ3:} %%CAMERA READY: \textit{Does ChatGPT demonstrate comparable effectiveness in detecting short-term changes in contemporary text and long-term changes in historical text?}\\

\begin{table}[!ht]
\centering
\caption{Macro-F1 scores obtained by SOTA systems, ChatGPT (best score), and BERT (last layer).}
%\caption{Comparison of (Macro-F1) scores obtained by SOTA systems on the full TempoWiC dataset and scores %obtained on our TempoWiC subset using the ChatGPT API, ChatGPT Web, and BERT. For ChatGPT API and Web, we report %the best score obtained in our experiments. For BERT, we report the score obtained using the last layer.}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{cc}
 & \textbf{Macro-F1} \\ \hline
\citealp{chen2022using} & .770 \\
\citealp{loureiro2022tempowic} & .703 \\
\citealp{loureiro2022tempowic} & .670 \\
\citealp{lyu2022mllabs} & .625 \\
\textit{ChatGPT API} & .689 \\
\textit{ChatGPT Web} & .580 \\
\textit{BERT} & .743 \\
\end{tabular}%
}
\label{tab:sota-tempowic}
\end{table}

Figures~\ref{fig:api-temperature} and~\ref{fig:web-prompt} show that ChatGPT's performance on TempoWiC is consistently lower than its performance on HistoWiC. In particular, in our experiments we observe that ChatGPT's performance ranges from .551 to .689 on TempoWiC and from .552 to .765 on HistoWiC. This suggests that ChatGPT is significantly more effective for long-term change detection than for short-term change detection. We believe that this might involve word meanings that were not explicitly covered during training, potentially allowing ChatGPT to detect anomalies from the usual patterns. We will further investigate this aspect in our future research.

For the sake of comparison, we report SOTA performance in Table~\ref{tab:sota-tempowic}. Results from this research are in italics.

\paragraph{RQ4:} %%CAMERA READY\textit{Can we enhance ChatGPT's performance in WiC tasks by raising the ``creativity'' using the temperature value?}\\

Figure~\ref{fig:api-temperature} shows that, on average, higher performance is associated with lower temperatures for both TempoWiC and HistoWiC, with accuracy decreasing as temperature values increase. Thus, we argue that high temperatures do not make it easier for  ChatGPT to solve WiC tasks or identify semantic changes effectively.

\paragraph{RQ5:} %%CAMERA READY\textit{Does ChatGPT API demonstrate comparable performance to ChatGPT Web in solving WiC tasks?}\\

ChatGPT Web results are presented in Table~\ref{tab:web}, along with the average performance we obtained through the ChatGPT API across temperature values ranging from 0.0 to 1.0 (API 0--1), from 1.0 to 2.0 (API 1--2), and from 0.0 to 2.0 (API 0--2). As with ChatGPT API, the performance of ChatGPT Web is higher for HistoWiC than for TempoWiC. In addition, our evaluation indicates that ChatGPT Web employs a moderate temperature setting, for we obtained consistent results when using a moderate temperature setting through ChatGPT API. This suggests that the ChatGPT API should be preferred  for solving downstream task like WiC. It also suggests that the current SOTA evaluations may achieve higher results if the official API were used instead of the web interface. \textbf{Thus, this implies that previous results using web interface should be interpreted with caution.}

\begin{table}[!ht]
\centering
\caption{Comparison of ChatGPT API and ChatGPT Web performance (Macro-F1)} %\caption{Comparison of ChatGPT Performance (Macro-F1) for TempoWiC and HistoWiC tasks using ChatGPT API and ChatGPT Web. We consider the average scores obtained over various temperatures as ChatGPT API values.}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
 & \multicolumn{4}{c}{\textbf{TempoWiC}} & \multicolumn{4}{c}{\textbf{HistoWiC}} \\ \cline{2-9} 
\multicolumn{1}{c|}{} & \textit{API} & \textit{API} & \textit{API} & \multicolumn{1}{c|}{\textit{web}} & \textit{API} & \textit{API} & \textit{API} & \multicolumn{1}{c|}{\textit{web}} \\
\multicolumn{1}{c|}{Temp.} & 0--1 & 1--2 & 0--2 & \multicolumn{1}{c|}{-} & 0--1 & 1--2 & 0--2 & \multicolumn{1}{c|}{-} \\ \hline
\multicolumn{1}{c|}{ZSp} & .609 & .589 & .600 & \multicolumn{1}{c|}{.580} & .713 & .665 & .688 & \multicolumn{1}{c|}{.686} \\
\multicolumn{1}{c|}{FSp} & .636 & .606 & .622 & \multicolumn{1}{c|}{.569} & .693 & .626 & .657 & \multicolumn{1}{c|}{.674} \\
\multicolumn{1}{c|}{MSp} & - & - & - & \multicolumn{1}{c|}{.500} & - & - & - & \multicolumn{1}{c|}{.565} \\ \hline
\multicolumn{1}{c|}{\textbf{all}} & .622 & .598 & .611 & \multicolumn{1}{c|}{.550} & .703 & .645 & .672 & \multicolumn{1}{c|}{.642}\\ \cline{2-9} 
\end{tabular}%
}
\label{tab:web}
\end{table}

\paragraph{RQ6:} %%CAMERA READY\textit{Can we enhance ChatGPT's performance in WiC tasks by providing it with a larger number of in-context examples?}\\

As shown in Figure~\ref{fig:web-prompt},  the performance of ChatGPT Web decreases as the number of example messages increases (from ZSp to MSp). This suggests that improving the performance of ChatGPT requires a more complex training approach than simply providing a few input-output examples. Furthermore, it indicates that the influence of message history is extremely significant in shaping the quality of conversations with ChatGPT. Indeed, a limited message history proved to be beneficial for the evaluation of ChatGPT API through FSp.

\paragraph{RQ7:} %%CAMERA READY\textit{Does ChatGPT outperform BERT embeddings in detecting semantic changes?} \\

Figure~\ref{fig:bert-layers} shows Macro-F1 scores obtained on TempoWiC and HistoWiC over the 12 BERT layers (see Appendix~\ref{app:bert}). When considering the final layer, which is conventionally used in downstream tasks, BERT obtains Macro-F1 scores of .750 and .743 for TempoWiC and HistoWiC, respectively. Similar to~\newcite{periti2023time}, BERT performs best on HistoWiC when embeddings extracted from middle layers are considered. However, BERT performs best on TempoWiC when embeddings extracted from the last layers are used. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{imgs/layers.png}
\caption{Comparison of BERT Performance (Macro-F1) for TempoWiC and HistoWiC tasks across layers}
\label{fig:bert-layers}
\end{figure}

We compared the performance of ChatGPT and BERT across their respective worst to best scenarios by sorting the Macro-F1 scores obtained by BERT and ChatGPT in ascending order (bottom x-axis). For ChatGPT, we consider the results obtained through FSp and ZSp prompting for TempoWiC and HistoWiC, respectively. As shown in Figure~\ref{fig:gptvbert}, even when considering the best setting, ChatGPT does not outperform the Macro-F1 score obtained by using the last layer of BERT, marked with a black circle. However, although it exhibits lower performance, the results obtained from ChatGPT are still comparable to BERT results on HistoWiC when embeddings extracted from the last layer of BERT are used.

\begin{figure}[!t]
\centering
\includegraphics[width=0.6\columnwidth]{imgs/gptvbert-nolabel.png}
\caption{ChatGPT v BERT (Macro-F1). Performance is sorted in ascending order regardless of temperatures and layers. A black circle denotes the use of the last layer of BERT.}%\caption{Comparison of BERT and ChatGPT performance (Macro-F1). Performance is sorted in ascending order regardless of temperatures and layers. For comparison, we marked  the performance of BERT when the last layer is used for embedding extraction with a black circle.}
\label{fig:gptvbert}
\end{figure}

Since our goal is to evaluate the potential of ChatGPT for recognizing lexical semantic changes, we analyzed the true negative rate and false negative rate scores, because \textit{negative} examples represent semantic change in TempoWiC and HistoWiC datasets. As shown in Figure~\ref{fig:tnrfnr}, regardless of the temperature and layer considered, ChatGPT falls short in recognizing semantic change for both TempoWiC and HistoWiC compared to BERT. However, it produces fewer false negatives than BERT for TempoWiC.\\

\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{imgs/tnrfnr.png}
\caption{True Negative Rate v False Negative Rate. Each cross represents a ChatGPT experiment. Each dot represents the use of a specific layer of BERT.}%\caption{True Negative Rate v False Negative Rate using ChatGPT and BERT. Each cross represents a ChatGPT experiment on TempoWiC and HistoWiC. Each dot represents the use of a specific layer of BERT on TempoWiC and HistoWiC}
\label{fig:tnrfnr}
\end{figure}

\paragraph{RQ8:} %%CAMERA READY\textit{Can we rely on the pretrained knowledge of ChatGPT to automatically solve the LSC task?}\\

In our experiment, ChatGPT achieved low Spearman’s correlation coefficients for each temperature when ranking the target word of the LSC English benchmark by degree of lexical semantic change. Higher correlations were achieved by using low temperatures rather than high ones (see Appendix~\ref{app:lsc}).
Table~\ref{tab:LSC} shows the ChatGPT correlation for the temperature 0. For comparison, we report correlations obtained by BERT-based systems that leverage pretrained models. Note that, when BERT is fine-tuned, it generally achieves even higher correlation scores (see survey by~\citealp{montanelli2023survey}).

\begin{table}[!ht]
\centering
\caption{LSC comparison: correlation obtained by SOTA BERT-based systems and ChatGPT (temperature=0).}
%\caption{Comparison of correlation obtained by SOTA BERT-based systems and correlation obtained by ChatGPT with temperature set to 0.}
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{cc}
 & \textbf{Spearman’s correlation} \\ \hline
\citealp{periti2023studying} & .651 \\ 
\citealp{laicher2021explaining} & .573 \\
\citealp{periti2022done} & .514 \\
\citealp{rother2020cmce} & .512 \\ 
\textit{ChatGPT API} & .251
\end{tabular}%
}
\label{tab:LSC}
\end{table}

As shown in Table~\ref{tab:LSC}, the BERT-based system largely outperforms ChatGPT, suggesting that ChatGPT is not currently well-adapted for use in solving LSC downstream tasks.

\subsection{BERT for Semantic Change Detection}
There are notable differences between the Macro-F1 for TempoWiC and HistoWiC in terms of how the results increase and decrease across layers (see Figure~\ref{fig:bert-layers}). For TempoWiC the results increase until the 8th layer, after which they remain almost stable. Conversely, for HistoWiC the BERT performance rapidly increases until the 5th layer, after which it linearly decreases until the 12th layer. As regards Tempo WiC, we hypothesize that BERT is already aware of the set of word meanings considered for evaluation as it was pretrained on modern and contemporary texts. As regards HistoWiC, we hypothesize that BERT is not completely aware of the set of word meanings considered for evaluation and that word representations adopted for the historical context of HistoWiC\footnote{1810--1860, as referenced in~\newcite{schlechtweg2020semeval}} might be slightly tuned. Thus, using medium embedding layers could prove beneficial in detecting semantic changes, as these layers are less affected by contextualization~\cite{ethayarajh2019contextual}. In other words, for HistoWiC, we hypothesize that the performance diminishes in the later layers due to the increasing contextualization of the medium and final embedding layers, which %hinders 
reduces the presence of noise in untuned word representations. This prompts us to question the appropriateness of using the last embedding layers to recognize historical lexical semantic change. We will address this question in  future research.

\section{Conclusion}
In this study, we empirically investigated the ability of ChatGPT to detect \textit{semantic change}. We used the TempoWiC benchmark to assess ChatGPT's ability to detect short-term semantic changes, and introduced a novel benchmark, HistoWiC, to assess ChatGPT's ability to recognize long-term changes. When considering the standard 12 layer of BERT, our experiments show that ChatGPT achieves comparable performance to BERT (although slightly lower) in regard to detecting long-term changes, but performs significantly worse in regard to recognizing short-term changes. We find that BERT's contextualized embeddings consistently provide a more effective and robust solution for capturing both short- and long-term changes in word meanings.

There are two possible explanations for the discrepancy in ChatGPT's performance between TempoWiC and HistoWiC: i) HistoWiC might involve word meanings not explicitly covered during training, potentially aiding ChatGPT in detecting anomalies; ii) TempoWiC involves patterns typical of Twitter (now X), such as abbreviations, mentions, or tags, which may render it more challenging than HistoWiC.

In light of our findings, we argue that \textit{ChatGPT might be the hero the world deserves but not the one it needs right now}, in particular for computationally modeling meaning over time, and by extension, for the study of semantic change.

\section*{Limitations}
Like all research on ChatGPT~\cite{laskar2023systematic, KOCON2023ChatGPT, zhong2023chatgpt}, our work has a significant limitation that we cannot address: our ChatGPT results are not entirely reproducible as ChatGPT is inherently nondeterministic. In addition, like ~\newcite{zhong2023chatgpt,jiao2023chatgpt}, we found that time and economic constraints when using ChatGPT dictated that our evaluation of the software had to be based on only  a subset of the TempoWiC and HistoWiC dataset. %Furthermore, due to time constraints, we conducted only a single experiment for each prompting strategy when considering ChatGPT by using the web interface. A more convincing approach would involve testing ChatGPT on a larger sample size and conducting multiple rounds of experiments for each temperature and prompt strategy. In future work, we aspire to not only evaluate ChatGPT on a broader range of examples but also to conduct more in-depth analysis and discussion across similar outputs at different temperatures.

In our study, we utilized ChatGPT 3.5. This could be considered a limitation, given the recent release of ChatGPT 4. However, we opted for ChatGPT 3.5 based on the guidance provided in the OpenAI documentation.\footnote{\url{https://platform.openai.com/docs/guides/gpt/which-model-should-i-use}} We acknowledge that OpenAI continues to train and release new models, which could potentially affect the reproducibility of our results.

One of the many features of ChatGPT is its ability to incorporate the history of preceding messages within a conversation while responding to new input prompts. However, there remain several unanswered questions regarding how this history influences the model's answers. This holds true even for the zero-shot prompting strategy, where a general setting is lacking. Multiple prompts can be provided as part of the same chat or across different chats. For simplicity, we assigned only one chat for each ZSp experiment. We intend to use different chats in our future work to examine and investigate the effect of the message history.

Finally, as highlighted by~\newcite{laskar2023systematic}, since the instruction-tuning datasets of OpenAI models are unknown (that is, not open source), the datasets used for evaluation may or may not be part of the instruction-tuning training data of OpenAI. 

Despite these limitations, we argue that our work is significant as it may prompt new discussion on the use of PFMs such as BERT and ChatGPT, while also dispelling the expanding belief that ChatGPT makes BERT an outdated technology.

\section*{Acknowledgements}
This work has in part been funded by the project Towards Computational Lexical Semantic Change Detection supported by the Swedish Research Council (2019–2022; contract 2018-01184), and in part by the research program Change is Key! supported by Riksbankens Jubileumsfond (under reference number M21-0021).

% CAMERA READY
%\section{Optional Supplementary Materials}
%Appendices or supplementary material (software and data) will be allowed ONLY in the final, camera-ready version, but not during submission, as papers should be reviewed without the need to refer to any supplementary materials.

%Each \textbf{camera ready} submission can be accompanied by an appendix usually being included in a main PDF paper file, one \texttt{.tgz} or \texttt{.zip} archive containing software, and one \texttt{.tgz} or \texttt{.zip} archive containing data.

%We encourage the submission of these supplementary materials to improve the reproducibility of results and to enable authors to provide additional information that does not fit in the paper. For example, preprocessing decisions, model parameters, feature templates, lengthy proofs or derivations, pseudocode, sample system inputs/outputs, and other details necessary for the exact replication of the work described in the paper can be put into the appendix. However, the paper submissions must remain fully self-contained, as these supplementary materials are optional, and reviewers are not even asked to review or download them. If the pseudo-code or derivations, or model specifications are an essential part of the contribution, or if they are important for the reviewers to assess the technical correctness of the work, they should be a part of the main paper and not appear in the appendix. Supplementary materials need to be fully anonymized to preserve the double-blind reviewing policy.


%APPENDIX
%Appendices are material that can be read and include lemmas, formulas, proofs, and tables that are not critical to the reading and understanding of the paper, as in \href{https://acl-org.github.io/ACLPUB/formatting.html#appendices}{*ACLPUB}. It is  highly recommended that the appendices should come after the references; the main text and appendices should be contained in a `single' manuscript file, without being separately maintained. Letter them in sequence and provide an informative title: \textit{Appendix A. Title of Appendix}


%\subsection{Extra space for ethical considerations and limitations}

%Please note that extra space is allowed after the 8th page (4th page for short papers) for an ethics/broader impact statement and a discussion of limitations. At submission time, if you need extra space for these sections, it should be placed after the conclusion so that it is possible to rapidly check that the rest of the paper still fits in 8 pages (4 pages for short papers). Ethical considerations sections, limitations, acknowledgments, and references do not count against these limits. For camera-ready versions, nine pages of content will be allowed for long (5 for short) papers.



